Relativistic Algebra of Space-Time and Algebrodynamics

We consider a manifestly Lorentz invariant form $\mathbb L$ of the biquaternion algebra and its generalization to the case of curved manifold. The conditions of $\mathbb L$-differentiability of $\mathbb L$-functions are formulated and considered as the primary equations for fundamental fields modeled with such functions. The exact form of the effective affine connection induced by $\mathbb L$-differentiability equations is obtained for the flat and curved cases. In the flat case, the integrability conditions of the latter lead to the self-duality of the corresponding curvature, thus ensuring that the source-free Maxwell and $SL(2,\mathbb C)$ Yang-Mills equations hold on the solutions of the $\mathbb L$-differentiability equations

==> GrginArXiv16.zip/preamble.tex <==
%% preamble.tex
%\documentclass[11pt,fleqn]{article}
\usepackage{amsfonts,amssymb,cite}
\usepackage{epsf,graphicx}

%\input preamble.tex
%\begin{document}
%\twocolumn[
%\jnumber{}{}

		%% PAGE SETUP AND TITLE BLOCK %%

\topmargin -10mm
\oddsidemargin -6mm
\evensidemargin -12mm
\textheight 242mm
\textwidth 178mm
\emergencystretch 6pt
\mathsurround 1pt
\mathindent 1em
\columnsep 8mm
\pagestyle{myheadings}
\newcommand{\bls}[1]{\renewcommand{\baselinestretch}{#1}}
\def\onecol{\onecolumn \mathindent 2em}
\def\twocol{\twocolumn \mathindent 1em}
\def\noi{\noindent}
\def\jnumber#1#2{\thispagestyle{empty} \noi\unitlength=1mm
    	\begin{picture}(178,10)
            \put(177,15){\llap{\large\it Grav. Cosmol. No.\,#1, #2}}
                    \end{picture}}

\newcommand{\Title}[1]{\noi {{\Large\bf #1}}\\[1ex]}

\newcommand{\Author}[2]{\noi{\bf #1}\\[2ex]\noi{\normalsize\it #2}\\}

\def\Aunames#1{\noi{\bf #1}}
\def\auth#1{${}^{#1}$}
\def\Addresses#1{\medskip\noi \protect
	\begin{description}\itemsep -3pt {\it #1} \end{description}}
\def\addr#1#2{\item[${}^{#1}$]{\it #2}}

\newcommand{\Rec}[1]{\noi {\it Received #1} \\}
\newcommand{\Recfin}[1]{\noi {\it Received in final form #1} \\}

\newcommand{\Abstract}[1]{\vskip 2mm \begin{center}
        \parbox{16.4cm}{\small\noi #1} \end{center}\medskip}
\newcommand{\PACS}[1]{\begin{center}{\small PACS: #1}\end{center}}
\newcommand{\foom}[1]{\protect\footnotemark[#1]}
\newcommand{\foox}[2]{\footnotetext[#1]{#2}\addtocounter{footnote}{1}}
\def\email#1#2{\footnotetext[#1]{e-mail: #2}\addtocounter{footnote}{1}}

\def\Talk{\foox 1 {Talk given at the International Conference RUSGRAV-14,
	   June 27 --- July 4, 2011, Ulyanovsk, Russia}}
\def\Plenary{\foox 1 {Plenary talk given at the International Conference 
	RUSGRAV-14, June 27 --- July 4, 2011, Ulyanovsk, Russia}}

		%%  TEXT AND SPACES %%

\def\nq{\hspace*{-1em}}
\def\nqq{\hspace*{-2em}}
\def\nhq{\hspace*{-0.5em}}
\def\nhh{\hspace*{-0.3em}}
\def\cm{\hspace*{1cm}}
\def\inch{\hspace*{1in}}
\def\wide{\mbox{$\dst\vphantom{\int}$}}
\def\Wide{\mbox{$\dst\vphantom{\intl_a^a}$}}
\def\ten#1{\mbox{$\cdot 10^{#1}$}}
\def\deg{\mbox{${}^\circ$}}                     %% degree
\def\degC{\mbox{${}^\circ$C}}                   %% Celsius degree
\def\Acknow#1{\subsection*{Acknowledgment} #1}

		%% FIGURES %%

\def\floatpagefraction{.95}
\def\topfraction{.95}
\def\bottomfraction{.95}
\def\textfraction{.05}
\def\dblfloatpagefraction{.95}
\def\dbltopfraction{.95}

\newcommand{\EFigure}[2]{\begin{figure} \centering   %% #1 = *.eps
        \framebox[85mm]{\epsfxsize=80mm\epsfbox{#1}} %% #2 = caption
        \caption{\protect\small #2}\medskip\hrule
	\end{figure}}
\newcommand{\REFigure}[2]{\begin{figure} \centering
        \framebox[85mm]{\epsfysize=80mm\rotate[r]{\epsfbox{#1}}}
        \caption{\protect\small #2}\medskip\hrule
	\end{figure}}
\newcommand{\WEFigure}[2]{\begin{figure*} \centering
        \framebox[178mm]{\epsfxsize=170mm\epsfbox{#1}}
        \caption{\protect\small #2}\medskip\hrule
	\end{figure*}}

		%% REFERENCES %%

\def\Jl#1#2{#1 {\bf #2},\ }

\def\ApJ#1 {\Jl{Astroph. J.}{#1}}
\def\CQG#1 {\Jl{Class. Quantum Grav.}{#1}}
\def\DAN#1 {\Jl{Dokl. AN SSSR}{#1}}
\def\GC#1 {\Jl{Grav. Cosmol.}{#1}}
\def\GRG#1 {\Jl{Gen. Rel. Grav.}{#1}}
\def\JETF#1 {\Jl{Zh. Eksp. Teor. Fiz.}{#1}}
\def\JETP#1 {\Jl{Sov. Phys. JETP}{#1}}
\def\JHEP#1 {\Jl{JHEP}{#1}}
\def\JMP#1 {\Jl{J. Math. Phys.}{#1}}
\def\NPB#1 {\Jl{Nucl. Phys. B}{#1}}
\def\NP#1 {\Jl{Nucl. Phys.}{#1}}
\def\PLA#1 {\Jl{Phys. Lett. A}{#1}}
\def\PLB#1 {\Jl{Phys. Lett. B}{#1}}
\def\PRD#1 {\Jl{Phys. Rev. D}{#1}}
\def\PRL#1 {\Jl{Phys. Rev. Lett.}{#1}}

		%% EQUATIONS %%

%% aligning, numbering
\def\al{&\nhq}
\def\lal{&&\nqq {}}
\def\eq{Eq.\,}
\def\eqs{Eqs.\,}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\bear{\begin{eqnarray}}
\def\bearr{\begin{eqnarray} \lal}
\def\ear{\end{eqnarray}}
\def\earn{\nonumber \end{eqnarray}}
\def\nn{\nonumber\\ {}}
\def\nnv{\nonumber\\[5pt] {}}
\def\nnn{\nonumber\\ \lal }
\def\nnnv{\nonumber\\[5pt] \lal }
\def\yy{\\[5pt] {}}
\def\yyy{\\[5pt] \lal }
\def\eql{\al =\al}
\def\eqv{\al \equiv \al}
\def\sequ#1{\setcounter{equation}{#1}}

%% fractions

\def\dst{\displaystyle}
\def\tst{\textstyle}
\def\fracd#1#2{{\dst\frac{#1}{#2}}}
\def\fract#1#2{{\tst\frac{#1}{#2}}}
\def\Half{{\fracd{1}{2}}}
\def\half{{\fract{1}{2}}}

%% other

\def\e{{\,\rm e}}
\def\d{\partial}
\def\re{\mathop{\rm Re}\nolimits}
\def\im{\mathop{\rm Im}\nolimits}
\def\arg{\mathop{\rm arg}\nolimits}
\def\tr{\mathop{\rm tr}\nolimits}
\def\sign{\mathop{\rm sign}\nolimits}
\def\diag{\mathop{\rm diag}\nolimits}
\def\dim{\mathop{\rm dim}\nolimits}
\def\const{{\rm const}}
\def\eps{\varepsilon}
\def\ep{\epsilon}

\def\then{\ \Rightarrow\ }
\newcommand{\toas}{\mathop {\ \longrightarrow\ }\limits }
\newcommand{\aver}[1]{\langle \, #1 \, \rangle \mathstrut}
\newcommand{\vars}[1]{\left\{\begin{array}{ll}#1\end{array}\right.}
\def\suml{\sum\limits}
\def\intl{\int\limits}

  %% Author's definitions

%\addtolength{\textheight}{1cm}
%\bls{1.0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{document}
%\thispagestyle{empty}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








